Approximate Propagation of both Epistemic and Aleatory Uncertainty through Dynamic Systems

When ignorance due to the lack of knowledge, modeled as epistemic uncertainty using Dempster-Shafer structures on closed intervals, is present in the model parameters, a new uncertainty propagation method is necessary to propagate both aleatory and epistemic uncertainty. The new framework proposed here, combines both epistemic and aleatory uncertainty into a second-order uncertainty representation which is propagated through a dynamic system driven by white noise. First, a finite parametrization is chosen to model the aleatory uncertainty by choosing a representative approximation to the probability density function conditioned on epistemic variables. The epistemic uncertainty is then propagated through the moment evolution equations of the conditional probability density function. This way we are able to model the ignorance when the knowledge about the system is incomplete. The output of the system is a Dempster-Shafer structure on sets of cumulative distributions which can be combined using different rules of combination and eventually transformed into a singleton cumulative distribution function using Smets' pignistic transformation when decision making is needed.

==> PolyChaos.tex <==
The problem in solving the mapping of DS structures as given in Eq.\eqref{mapping} is to find $Y=[\underline{y},\overline{y}]$ such that:
%
\begin{eqnarray}
Y = f(A, B) \label{IntProp}
\end{eqnarray}
%
where $ A = [\underline{a},\overline{a}]$ and $B = [\underline{b},\overline{b}]$. While in this paper we present only the bivariate case, the method can be scaled to the desired number of variables. 

The problem can be transformed into finding the stochastic response $y$ by defining $a \sim \mathcal{U}(\underline{a},\overline{a})$ and $b \sim \mathcal{U}(\underline{b},\overline{b})$:
%
\begin{eqnarray}
y = f(a, b)
\end{eqnarray}
%
and write the polynomial chaos expansion for the uncertain arguments and the response:
%
\begin{eqnarray}
a = \sum_{i=0}^{p-1} a_i \psi_i(\xi_1) \quad \mathrm{where} \quad \xi_1 \sim \mathcal{U}(-1,1) \\
b = \sum_{j=0}^{p-1} b_j \psi_j(\xi_2) \quad \mathrm{where} \quad \xi_2 \sim \mathcal{U}(-1,1) \\
y = \sum_{k=0}^{P-1} y_k \bm{\psi}_k(\bm{\xi}) \quad \mathrm{where} \quad P = \frac{(n+p)!}{n!p!} \label{responsePC}
\end{eqnarray}

For this paper we are only concerned with the Uniform distribution, however due to the specificity of this application any other probability distribution with compact support can be used (Eq. Beta).

Here $n$ is the number of uncertain input variables and $p$ the order of the polynomial chaos expansion. The basis function $\psi_n$ is the $n$-th degree Legendre polynomial and the polynomial coefficients of the input variables are given by:
%
\begin{eqnarray}
a_0 = \frac{\overline{a}+\underline{a}}{2} ~,~ a_1 = \frac{\overline{a}-\underline{a}}{2} ~,~ a_2 = \ldots = a_{p-1} = 0 \\
b_0 = \frac{\overline{b}+\underline{b}}{2} ~,~ b_1 = \frac{\overline{b}-\underline{b}}{2} ~,~ b_2 = \ldots = b_{p-1} = 0 
\end{eqnarray}

The first six multidimensional Legendre polynomials for the bivariate case are given by:
%
\begin{eqnarray}
\bm{\psi}_0(\bm{\xi}) &= \psi_0(\xi_1)\psi_0(\xi_2) &= 1 \\
\bm{\psi}_1(\bm{\xi}) &= \psi_1(\xi_1)\psi_0(\xi_2) &= \xi_1 \\
\bm{\psi}_2(\bm{\xi}) &= \psi_2(\xi_1)\psi_0(\xi_2) &= \frac{1}{2}(3\xi_1^2-1) \\
\bm{\psi}_3(\bm{\xi}) &= \psi_0(\xi_1)\psi_1(\xi_2) &= \xi_2 \\
\bm{\psi}_4(\bm{\xi}) &= \psi_1(\xi_1)\psi_1(\xi_2) &= \xi_1 \xi_2 \\
\bm{\psi}_5(\bm{\xi}) &= \psi_2(\xi_1)\psi_1(\xi_2) &= \frac{1}{2}(3\xi_1^2-1) \xi_2
\end{eqnarray}

We are interested in finding the polynomial coefficients $y_k$ which characterize the stochastic behavior of the output variable. Using the Galerkin projection and the orthogonality property of the polynomials one can isolate the coefficients $y_k$ as shown in Ref. \cite{Eldred2008}:
%
\begin{eqnarray}
y_k = \frac{<f,\bm\psi_k>}{<\bm\psi_k^2>} = \frac{1}{<\bm\psi_k^2>} \int_\Omega f \psi_k \varsigma(\bm\xi) \mathrm{d}\bm\xi
\end{eqnarray}
%
where $\varsigma(\bm\xi) = \prod_{i=1}^n \varsigma_i(\xi_i)$ is the joint probability density function. The integral can be evaluated using sampling or quadrature techniques.

We show that by bringing the polynomial chaos expansion to a Bernstein form using the Garloff's method \cite{Garloff1985}, we can efficiently find the minimum and the maximum value of the compact support thanks to the properties of the Bernstein polynomials: the smallest and the largest coefficient bound the output of the function modeled.

To transform our expansion from Legendre polynomial basis to Bernstein polynomial basis we expand our Polynomial Chaos expansion, Eq.\eqref{responsePC} into a simple power series and identify the new coefficients.
%
\begin{eqnarray}
y = \sum_{\mathbf{I} \le \mathbf{N}} \alpha_\mathbf{I} \bm\xi^\mathbf{I} \label{powerSeries}
\end{eqnarray}
%
where the multi-index $\mathbf{I} = (i_1, \ldots, i_n) \in \mathbb{N}^n$ and $\mathbf{N} = (n_1, \ldots, n_n) \in \mathbb{N}^n$ is the multi-index of maximum degrees, thus the maximum degree of $\xi_k$ is given by $n_k$. Here, we denote $\bm\xi^I = \xi_1^{i_1} \cdot \ldots \cdot  \xi_n^{i_n}$ and the inequality $\mathbf{I} \le \mathbf{J}$ implies $i_1 \le j_1, \ldots, i_n \le j_n$.


==> RespAgg.tex <==
If two or more experts have belief about a model parameter, their belief can be combined from the outset using the Dempster rule of combination, Eq.\eqref{DempsterRule}, then the procedure follows as described in subsections \ref{sec:Moments}-\ref{sec:DMDSPS}.

When experts do not agree on a particular model, then the result is a collection of competing models as described in Eq.\eqref{compete1}-\eqref{compete2}. The DS structure over p-boxes obtained from each model can be aggregated using the Dempster rule of combination, Eq.\eqref{DempsterRule}, for every $x_f$ to obtain a new DS structure for the response of the system, $P(X \le x_f | \mathbf{e}_0)$,
%
\begin{eqnarray}
m_{1\oplus 2}[P(X \le x_f | \mathbf{e}_0)] = m_1[P(X \le x_f | \mathbf{e}_0)] \oplus m_2[P(X \le x_f | \mathbf{e}_0)]
\end{eqnarray}

Here, $\oplus$ represents the rule for the combination of evidence provided by the two models. No model uncertainty is considered in this paper, and both models are considered equally reliable. However, when the reliability of the models is available or the models offer conflicting evidence about the response of the system a discounting function can be used in combining the two sources of information \cite{Sentz2002}.

The result is a DS structure similar with the one in Eq.\eqref{finalDS}, which can be used for risk assessment or decision making. A general view on evidence combination when competing models exists is presented in  Fig.\ref{fig:combined}.

\begin{figure}
	\centering
		\includegraphics[width=5in]{imgs/combined.eps}
		\caption{Response aggregation}
	\label{fig:combined}
\end{figure}

While in this paper, we have presented just the Dempster rule of combination, which is a generalization of the Bayes rule, other combinations rules \cite{Sentz2002} are available which treat the conflicting evidence differently. The Dempster rule of combination emphasizes only the agreement between sources and ignores all the conflicting evidence. This is particularly worrisome when dealing with approximate uncertainty propagation which may result in artificial conflicting evidence due to assumptions about the class of distributions to represent the uncertainty in the aleatory variables. This problem remains to be thoroughly address in a future study.

==> evidence.tex <==
The Dempster-Shafer structure about a variable $x$ is identified by the basic probability assignment (bpa), denoted here by $m$, which is similar to the probability in the probability theory. The bpa for a given set can be understood as the weight of evidence that the truth is in that set, evidence, which cannot be further subdivided. It defines a map of the power set over the \textit{frame of discernment} $\Omega$ to the interval $[0,1]:$ $m[x]:2^\Omega \rightarrow [0,1]$. The \textit{focal element} of $m$ is every subset $A \subseteq \mathbb{R}$ such that $m[x](A)>0$ and the \textit{belief structure} $m$ verifies:
%
\begin{eqnarray}
\sum_{A \subseteq \Omega} m[x](A) = 1 \quad \mathrm{where} \quad m[x](A_i) = p_i
\end{eqnarray} 

In this work we are considering only focal elements as closed intervals, $A = [\underline{A} , \overline{A}]$ , and normalized belief structures (closed-world assumption) which satisfy the following relation: $m(\phi)=0$, where $\phi$ is the null set.

Based on the mass function two new functions can be induced. The \textit{belief function} or the \textit{lower bound}, $Bel$, which quantifies the total amount of support given to the set of interest $A$:
%
\begin{eqnarray}
Bel[x](A) = \sum_{B \subseteq A} m[x](B)
\end{eqnarray} 	

The \textit{plausibility function} or the \textit{upper bound}, $Pl$, which quantifies the maximum amount of potential given to the set of interest $A$ (here $\bar{A}$ is the complement of $A$):
%
\begin{eqnarray}
Pl[x](A) = \sum_{B \cap A \neq \phi} m[x](B) = 1 - Bel[x](\bar{A})
\end{eqnarray} 	

The precise probability is bounded by the two quantities defined above, and when the equality is satisfied then the belief measures is just a probability measure and all the focal elements are singletons.
%
\begin{eqnarray}
Bel[x](A) \le P(x \in A) \le Pl[x](A)
\end{eqnarray} 	

Given the two functions defined above one can define the \textit{degree of ignorance} as the difference between plausibility and belief \cite{Biondo1990}, which is the amount of belief which cannot be committed to $A$ nor to its complement, $\bar{A}$.
%
\begin{eqnarray}\label{ignorance}
Ig[x](A) = Pl[x](A) - Bel[x](A) = 1 - \left( Bel[x](A) + Bel[x](\bar{A}) \right)
\end{eqnarray} 	

Given two bpa's $m_1$ and $m_2$ based on independent arguments on the same frame of discernment, the Dempster's rule of combination provides the means to calculate the aggregation of the two belief structures:
%
\[ \label{DempsterRule}
m_{1\oplus 2}[x](A) =\left \{
\begin{array}{cc}
    \frac{1}{1-K} \sum_{B \cap C = A} m_1[x](B) m_2[x](C), & \mathrm{for}~A \neq \phi \\
    0, & \mathrm{otherwise} \\
\end{array}
\right.  \\
\]
%
where $K = \sum_{B \cap C = \phi} m_1[x](B) m_2[x](C)$ represents the amount of probability mass due to conflict.

To be able to use the traditional normative decision theory based on the expected utility, one needs that the probability of each singleton in the frame of discernment has to be defined. Smets \cite{Smets1990} shows how to make decisions using the belief functions by constructing a unique transformation between the belief function and the probability function. This transformation is called the \textit{pignistic transformation} and it distributes the basic probability assignment equally among each singleton element once decisions have to be made.
%
\begin{eqnarray} \label{pignistic}
BetP[x](A) = \sum_{B \subseteq \Omega} m[x](B) \frac{|A \cap B|}{|B|}
\end{eqnarray} 	

Here $|\cdot|$ is the cardinality of the set. The probability function $BetP$ can be used to make decisions with the expected utility theory.


==> framework.tex <==
Consider the following 1-dimensional linear dynamical system driven by noise and with uncertain initial conditions modeled using a Gaussian pdf:
%
\begin{eqnarray}
x_{k+1} &=& \alpha x_k + w_k \\
p(t_0, x_0) &=& \mathcal{N}(x_0|\mu_0,\sigma_0^2)
\end{eqnarray}

The process noise $w_k$ is temporally uncorrelated, zero-mean random sequence with known variance, $q_k$. We are interested in the response of the system after $N$ steps when the parameter $\alpha$ is uncertain and modeled using a DS structure on the closed interval, $[\underline{\alpha},\overline{\alpha}]$.

Since all the random variables are modeled using Gaussian distributions and the dynamical system is linear with additive noise, the stochastic response of the system is guarantee to have a Gaussian distribution. The evolution of the two moments are given by \cite{Kalman1960}:
%
\begin{eqnarray}\label{lin_syst}
\mu_{k+1} = \alpha \mu_k \\
\sigma^2_{k+1} = \alpha^2 \sigma^2_k + q_k
\end{eqnarray}

In Ref.\cite{Chen1997} it is shown that the same relations are valid for interval representation of the variables. Thus given $\alpha \in \alpha^I = [\underline{\alpha},\overline{\alpha}]$, at time $t_k$ we obtain $\mu_k \in \mu_k^I = [\underline{\mu_k},\overline{\mu_k}]$ and $\sigma^2_k \in {\sigma^2_k}^I = [\underline{\sigma^2_k},\overline{\sigma^2_k}]$. If there is a belief structure over $\alpha$ we obtain a 2-tuple for each focal element in the DS-structure. This way we obtain a DS-structure over probability sets as described in Section \ref{sec:ProbSets}.

Here we have presented epistemic uncertainty in the parameter of the dynamical system. However, without loss of generality, this approach can be extended to any other variable existing in the Eq.\eqref{lin_syst}. We may be ignorant about the characterization of the prior distribution or the process noise. If two or more experts have belief about a parameter, their belief can be combined from the outset using the Dempster rule of combination then the procedure follows as described above.

Using the mapping described in Section \ref{sec:Mapping}, the same approach can be extended to nonlinear dynamical systems. Moreover we may have experts that do not agree on a particular model, thus the DS-structure over p-boxes can accommodate the aggregation of their beliefs as exemplified in Fig.\ref{fig:framework} even in the presence of conflict.

%\begin{figure}
%	\centering
%		\includegraphics[width=5in]{imgs/framework.eps}
%		\caption{Nonlinear Data Assimilation with Ignorance}
%	\label{fig:framework}
%\end{figure}
 

==> garloff.tex <==
We are interested in the transformation of the power series in Eq.\eqref{powerSeries} into its Bernstein form:
%
\begin{eqnarray}
y = \sum_{\mathbf{I} \le \mathbf{N}} \beta_\mathbf{I} \mathbf{B}_{\mathbf{I}}^{\mathbf{N}}(\bm\xi) \label{bernExpansion}
\end{eqnarray}
%
where $\mathbf{B}_{\mathbf{I}}^{\mathbf{N}}(\bm\xi)$ is the $\mathbf{I}$th Bernstein polynomial of degree $\mathbf{N}$ on the general box $G = [\underline{\bm\xi}, \overline{\bm\xi}]$. In our bi-variate case $G = [-1,1] \times [-1,1]$ since $\xi_1, \xi_2 \sim \mathcal{U}(-1,1)$.
%
\begin{eqnarray}
\mathbf{B}_{\mathbf{I}}^{\mathbf{N}}(\bm\xi) = B_{i_1}^{n_1}(\xi_1) \cdot \ldots \cdot B_{i_n}^{n_n}(\xi_n)
\end{eqnarray}
%
where the univariate Bernstein polynomial $B_k^n(\xi)$ on the general interval $[\underline{\xi}, \overline{\xi}]$ is given by:
%
\begin{eqnarray}
B_k^n(\xi) = {n \choose k} \frac{(\xi-\underline{\xi})^k(\overline{\xi}-\xi)^{n-k}}{(\overline{\xi}-\underline{\xi})^n}
\end{eqnarray}

The Bernstein coefficients $\beta_{\mathbf{I}}$ are given by:
%
\begin{eqnarray}
\beta_{\mathbf{I}} = \sum_{\mathbf{J} \le \mathbf{I} \le \mathbf{N}} \frac{{\mathbf{I} \choose \mathbf{J}}}{{\mathbf{N} \choose \mathbf{J}}} \hat{\alpha}_{\mathbf{J}} \label{bernCoeff}
\end{eqnarray}
% 
where we write ${\mathbf{I} \choose \mathbf{J}} = {i_1 \choose j_1} \cdot \ldots \cdot {i_n \choose j_n}$.

The scaled coefficients $\hat{\alpha}_{\mathbf{I}}$ are obtained as described in Ref.\cite{Berchtold2000} from the $\alpha_{\mathbf{I} }$ coefficients in Eq.\eqref{powerSeries} and the box $G$:
%
\begin{eqnarray}
\hat{\alpha}_{\mathbf{I}} &=& \tilde{\alpha}_\mathbf{I}(\overline{\bm\xi} - \underline{\bm\xi})^\mathbf{I} \label{finalCoeff} \\
\tilde{\alpha}_\mathbf{I} &=& \sum_{\mathbf{I} \le \mathbf{J} \le \mathbf{N}} {\mathbf{J} \choose \mathbf{I}} \alpha_\mathbf{J} \underline{\bm\xi}^{\mathbf{J}-\mathbf{I}} \label{interCoeff}
\end{eqnarray}

\textit{Example}: Consider the following Polynomial Chaos expansion given by $n=2, p=3$ and $P=10$:
%
\begin{eqnarray}
y = 5\bm{\psi}_0(\bm{\xi}) + \bm{\psi}_1(\bm{\xi}) + \bm{\psi}_3(\bm{\xi}) + \bm{\psi}_4(\bm{\xi}) \nonumber
\end{eqnarray}

Transforming this expansion into a simple power series we obtain the folowing polynomial:
%
\begin{eqnarray}
y = 5 + \xi_1 + \xi_2 + \xi_1 \xi_2 \nonumber
\end{eqnarray}
%
where $a_{00} = 5, a_{10} = 1, a_{01} = 1$, and $a_{11} = 1$. Here the multi-index of maximum degree is $\mathbf{N} = (1,1)$.

The following intermediate coefficients are obtain from Eq.\eqref{interCoeff} in order to perform the scaling operation: $\tilde{a}_{00} = 4, \tilde{a}_{01} = 0, \tilde{a}_{10} = 0$, and $\tilde{a}_{11} = 1$. The final set of power-coefficients is given by Eq.\eqref{finalCoeff}: $\hat{a}_{00} = 4, \hat{a}_{01} = 0, \hat{a}_{10} = 0$, and $\hat{a}_{11} = 4$.

Finally, the Bernstein coefficients are obtain using Eq.\eqref{bernCoeff}: $\beta_{00} = 4, \beta_{01} = 4, \beta_{10} = 4$, and $\beta_{11} = 8$, and the Bernstein basis is given by:
%
\begin{eqnarray}
\mathbf{B}_{00}^{11} &= \frac{1}{16}(1-\xi_1)(1-\xi_2) \quad \mathbf{B}_{01}^{11} &= \frac{1}{16}(1-\xi_1)(\xi_2+1) \nonumber \\
\mathbf{B}_{10}^{11} &= \frac{1}{16}(\xi_1+1)(1-\xi_2) \quad \mathbf{B}_{11}^{11} &= \frac{1}{16}(\xi_1+1)(\xi_2+1) \nonumber
\end{eqnarray}

==> range.tex <==
Given the Bernstein expansion in Eq.\eqref{bernExpansion}, the range enclosing property \cite{Garloff1993} gives a bound on the polynomial in terms of the Bernstein coefficients:
%
\begin{eqnarray}
\min_{\mathbf{I} \le \mathbf{N}} \beta_{\mathbf{I}} \le y(\bm\xi) \le \max_{\mathbf{J} \le \mathbf{N}} \beta_{\mathbf{J}} \quad \forall ~ \bm\xi \in G = [\underline{\bm\xi}, \overline{\bm\xi}]
\end{eqnarray}

Provided that the initial box is small enough, the range provided by the Bernstein form is exact. Compared with other forms in estimating the range, it is experimentally shown in Ref. \cite{Stahl1995} that the Bernstein form provides the smallest average overestimation error in the univariate case.

Tighter bounds can be obtained by subdivision of the initial box and choosing the minimum and the maximum of all the Bernstein coefficients corresponding to each sub-box. An efficient algorithm for range computation that incorporates a number of features such as subdivision, cut-off test, simplified vertex test, monotonicity test and others is provided in Ref.\cite{Ray2008}.

Therefore, getting back to our problem in mapping DS structures on closed intervals Eq.\eqref{mapping} and Eq.\eqref{IntProp} the output interval or the focal element $Y=[\underline{y},\overline{y}]$ is given by:
%
\begin{eqnarray}
\underline{y} = \min_{\mathbf{I} \le \mathbf{N}} \beta_{\mathbf{I}} \quad \mathrm{and} \quad \overline{y} = \max_{\mathbf{J} \le \mathbf{N}} \beta_{\mathbf{J}}
\end{eqnarray}

This methodology is applied to map all the focal elements in the initial body of evidence through the nonlinear function. Their corresponding masses are obtained using Eq.\eqref{mapping}. This way a body of evidence for the response is constructed.
